BEhavioral Leakage and IntEr-cycle Variability Emulator model for ReRAMs (BELIEVER)

Emerging electronic devices are promising to drive the performance of computer systems to new heights, against the notable saturation in traditional transistor-based architectures. Among them, resistive RAM -- or ReRAM -- has attracted a lot of attention among scientists since its practical realization was reported in 2008 and numerous devices, circuits and systems, and also models have been described in the literature. However, behavioral models fail to reproduce device parameter variations and the drift of device state in the absence of a stimulus. This shortcoming substantially reduces the practical relevance of systems and circuits designed with existing models. The work at hand deals with the development of a behavioral model that integrates device parameter variation and state drift based on data collected from our measurements of real devices. As we show in this paper, BELIEVER model enables engineers to conduct more reliable and meaningful design and simulations of circuits and systems that use ReRAMs.

==> figures/img/src/basic_elements.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage[utf8]{inputenc}
%\usepackage[europeanresistors]{circuitikz}

%\usetikzlibrary{positioning}
\newcommand*{\equal}{=}
\def\xlen{4mm}

%\begin{document}
    \begin{circuitikz}
        \draw (0,0) node(right1){} to[resistor, l_=$v\equal R\cdot i$, o-o]+(-4,0) node(left1){};
        \draw (left1) to[capacitor, l_=$q\equal C\cdot v$, o-o]+(0,-4) node(bottomleft){};
        \draw (right1) to[inductor, l^=$\phi \equal L\cdot i$, o-o]+(0,-4) node(bottomright){};
        \draw (bottomleft) to[memristor, l_=$\phi \equal M\cdot q$, o-o]+(4,0);
        
        \draw (left1) to[short, l_=$\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ } u\equal -\frac{\partial \phi}{\partial t}$, o-o]+(4,-4);
        \draw (right1) to[short, l_=$\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ }\textnormal{ } i\equal \frac{\partial q}{\partial t}$, o-o]+(-4,-4);
        
        \draw (-4.5,0.5) node(vol){Voltage};
        \draw (-4.5,-4.5) node(cha){Charge};
        \draw (0.3,-4.5) node(flu){Flux};
        \draw (0.4,0.5) node(cur){Current};
    \end{circuitikz}
%\end{document}

==> figures/img/src/measurementsetup.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage[utf8]{inputenc}
%\usepackage[europeanresistors]{circuitikz}

%\usetikzlibrary{positioning}

\def\xlen{4mm}

%\begin{document}
    \begin{circuitikz}
       \draw (4,2) node[buffer](opv1){$G_\mathrm{Y}\textnormal{ }$};
       %\draw (opv1.+) -- +(0,-0.5)node[rground]{};
       \draw (opv1.in) to[memristor,l_=$M$, -]+(-3,0) node(input){};

       %\draw (opv1.-) to[short, *-] +(0,1.5) to[R,l=$R_F$]+(3,0) to[short, -] +(0.1,0) to[short, -*] +(0,-2) to[short, -] (opv1.out);
       \draw (opv1.out) to[short, -o] +(0.5,0) node(output){};
       \draw (input) to[short,*-]+(0,0) node(input2){};
       \draw (input2) to[esource,l_=$V_\mathrm{in}$]+(0,-4) node(ground2){};
       \draw (ground2) node[rground]{};
       
       \draw (input) to[short, -]+(0,1.5) node(node1){};
       \draw (node1) to[short, -]+(6.4,0) node(node2){};
       \draw (opv1.out)+(0.55,0) to[short, -*]+(2,0) node(node3){};
       \draw (node3) to[short, -*]+(0,-1.5) node(node4){};
       \draw (node4) to[short, -]+(0,-1.5) node(node5){};
       \draw (node2) to[oscope,l_=$Ch1$, -]+(2,0) node(ch1){};
       \draw (node3) to[oscope,l_=$Ch2$, -*]+(2,0) node(ch2){};
       \draw (node4) to[oscope,l_=$Ch3$, -*]+(2,0) node(ch3){};
       \draw (node5) to[oscope,l_=$Ch4$, -*]+(2,0) node(ch4){};
       \draw (ch1) to[short, -]+(0,-5.5) node(ground3){};
       \draw (ch4)+(0,-1) node[rground]{};
       
       %Spannungspfeile
       %\node at (-0.3,1.3) {$V_{in}$};
       %\draw[-latex,line width=0.3pt] (input) -- +(0, -1.4);
       %\draw (input) +(0,-2)node[rground]{} to[short, -] +(0,-1.5); 
       
       \node at (4.7,0) {$V_\mathrm{out}$};
       \draw[-latex,line width=0.3pt] (opv1.out) +(0.5,-0.1) -- +(0.5, -3.9);
       \draw (opv1.out) +(0.5,-4) node[rground]{} to[short, o-] +(0.5,-4); 
    \end{circuitikz}
%\end{document}

==> figures/img/src/measurementsetup_2.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage[utf8]{inputenc}
%\usepackage[europeanresistors]{circuitikz}

%\usetikzlibrary{positioning}

\def\xlen{4mm}

%\begin{document}
    \begin{circuitikz}[scale = 0.7]
       
       \draw (4,2) node[op amp](opv1){};
       \draw (opv1.+) -- +(0,-0.5)node[rground]{};
       \draw (opv1.-) to[memristor,l_=$M$, -*]+(-3,0) node(input){};
       \draw (input) to[short,-o] +(-1.5,0) node(vauin){};

       \draw (opv1.-) to[short, *-] +(0,1.5) to[R,l=$R_\mathrm{F}$]+(3.3,0) to[short, -] +(0,-0.2) to[short, -*] +(0,-2) to[short, -] (opv1.out);
       \draw (opv1.out) to[short, -] +(2,0) node(opvout){};
       
       \draw (input) to[short, *-]+(0,3) node(node1){};
       \draw (node1) to[short, -]+(8.4,0) node(node2){};
       
       \draw (opvout) to[short, -*]+(0,0) node(node3){};
       \draw (node3) to[short, -*]+(0,-2.2) node(node4){};
       \draw (node4) to[short, -]+(0,-2.2) node(node5){};
       \draw (node2) to[oscope,l_=$Ch1$, -]+(2,0) node(ch1){};
       \draw (node3) to[oscope,l_=$Ch2$, -*]+(2,0) node(ch2){};
       \draw (node4) to[oscope,l_=$Ch3$, -*]+(2,0) node(ch3){};
       \draw (node5) to[oscope,l_=$Ch4$, -*]+(2,0) node(ch4){};
       \draw (ch1) to[short, -]+(0,-10) node(ground3){};
       \draw (ch4)+(0,-1.5) node[rground]{};
       
       %Spannungspfeile
       \node at (-1.7,1.9) {$V_\mathrm{in}$};
       \draw[-latex,line width=0.3pt] (vauin) -- +(0, -1.3);
       \draw (vauin) +(0,-1.5)node[rground]{} to[short, o-] +(0,-1.5); 
       
       \node at (6.2,1.4) {$V_\mathrm{out}$};
       \draw[-latex,line width=0.3pt] (opv1.out) +(-0.1,-0.2) -- +(-0.1, -1);
       \draw (opv1.out) +(-0.1,-1.2) node[rground]{} to[short, o-] +(-0.1,-1.2); 
       
       
       
    \end{circuitikz}
%\end{document}

==> figures/img/src/transimpedanceamplifier.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage[utf8]{inputenc}
%\usepackage[europeanresistors]{circuitikz}

%\usetikzlibrary{positioning}

\def\xlen{4mm}

%\begin{document}
    \begin{circuitikz}
       \draw (4,2) node[op amp](opv1){};
       \draw (opv1.+) -- +(0,-0.5)node[rground]{};
       \draw (opv1.-) to[memristor,l_=$M$, -o]+(-3,0) node(input){};

       \draw (opv1.-) to[short, *-] +(0,1.5) to[R,l=$R_\mathrm{F}$]+(3,0) to[short, -] +(0.1,0) to[short, -*] +(0,-2) to[short, -] (opv1.out);
       \draw (opv1.out) to[short, -o] +(2,0);
       
       %Spannungspfeile
       \node at (-0.5,1.8) {$V_\mathrm{in}$};
       \draw[-latex,line width=0.3pt] (input) -- +(0, -1.4);
       \draw (input) +(0,-1.5)node[rground]{} to[short, o-] +(0,-1.5); 
       
       \node at (7.6,1.5) {$V_\mathrm{out}$};
       \draw[-latex,line width=0.3pt] (opv1.out) +(2,-0.1) -- +(2, -0.9);
       \draw (opv1.out) +(2,-1) node[rground]{} to[short, o-] +(2,-1); 
       
       
       
    \end{circuitikz}
%\end{document}

==> figures/img/src/voltagedivider.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage[utf8]{inputenc}
%\usepackage[europeanresistors]{circuitikz}

%\usetikzlibrary{positioning}

\def\xlen{4mm}

%\begin{document}
    \begin{circuitikz}
        \draw (2,2) node(ground1){} to[resistor,l_=$R_\mathrm{S}$, -*]+(0,4) node(out){};
        \draw (2,2) node[rground]{};
        \draw (out) to[memristor,l_=$M$, -o]+(0,4) node(input){};
        \draw (out) to[short,-o] +(2,0);
       
      %Spannungspfeile
      
        \draw (out)+(-2,0) node(dummy1){$V_\mathrm{in}$};
        \draw[-latex,line width=0.3pt] (input)+(-1.5,0) -- +(-1.5, -8.3);
        
        \draw[-latex,line width=0.3pt] (out)+(2,-0.20) -- +(2, -4.3);
        \draw (out)+(2.5,-2) node(dummy1){$V_\mathrm{out}$};
       
       
       
    \end{circuitikz}
%\end{document}

==> figures/img/src/voltdivider_horiz.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage[utf8]{inputenc}
%\usepackage[europeanresistors]{circuitikz}

%\usetikzlibrary{positioning}

\def\xlen{4mm}

%\begin{document}
    \begin{circuitikz}
        \draw (2,2) node(ground1){} to[resistor,l_=$R_\mathrm{S}$, -*]+(-4,0) node(out){};
        \draw (2,2) node[rground]{};
        \draw (out) to[memristor,l_=$M$, -o]+(-4,0) node(input){};
        \draw (out) to[short,-o] +(0,1);
       
      %Spannungspfeile
      
        \draw (out)+(0,-1.1) node(dummy1){$V_\mathrm{in}$};
        \draw[-latex,line width=0.3pt] (input)+(0,-0.7) -- +(8, -0.7);
        
        \draw[-latex,line width=0.3pt] (out)+(0.2,1) -- +(4, 1);
        \draw (out)+(2,1.3) node(dummy1){$V_\mathrm{out}$};
       
       
       
    \end{circuitikz}
%\end{document}

==> setups/ACMsetup.tex <==
\usepackage[utf8]{inputenc}

%\citestyle{acmauthoryear}
\usepackage{booktabs} % For formal tables

\usepackage[ruled]{algorithm2e} % For algorithms

% Metadata Information
\acmJournal{TCPS}
% \acmVolume{9}
% \acmNumber{4}
% \acmArticle{39}
 \acmYear{2018}
% \acmMonth{3}

%\acmBadgeL[http://ctuning.org/ae/ppopp2016.html]{ae-logo}
%\acmBadgeR[http://ctuning.org/ae/ppopp2016.html]{ae-logo}

% Copyright
\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
%\setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}

% DOI
\acmDOI{0000001.0000001}

%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below.
%

% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%
% End generated code
%




==> text/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Health-care (alphabetic order):							   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{asd}{ASD}{Autism Spectrum Disorder}
\newacronym{cart}{CART}{Classification And Regression Tree}
\newacronym{dfa}{DFA}{Discriminant Function Analysis} 
\newacronym{ecg}{ECG}{Electrocardiography}
\newacronym{skin_eda}{EDA}{Electrodermal activity} 		
%In conflict with SoC definition
\newacronym{ews}{EWS}{Early Warning Score}
\newacronym{ga}{GA}{Genetic Algorithm}
\newacronym{hr}{HR}{Heart Rate}
\newacronym{ldf}{LDF}{Linear Discriminant Function}
\newacronym{rmsdd}{RMSDD}{Root-Mean Square of Successive Differences}
\newacronym{rsvm}{RSVM}{Reputation-driven Support Vector Machine }
\newacronym{saews}{SA-EWS}{Self-Aware Early Warning Score}
\newacronym{sam}{SAM}{Self-Assessment Manikin} 
\newacronym{selphys}{SelPhyS}{Self-aware cyber-Physical System}
\newacronym{sdnn}{SDNN}{Standard Deviation Normal-to-Normal-Intervals}
\newacronym{skt}{SKT}{Skin Temperature}
\newacronym{som}{SOM}{Self-Organizing Map}
\newacronym{whs}{WHS}{Wearable Health-care Systems}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Learning:													   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{ann}{ANN}{Artificial Neural Network}
\newacronym{bpn}{BPN}{Back-Propagation Neural Network}
\newacronym{bpnn}{BPNN}{back-propagation neural network}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{flop}{FLOP}{Floating Point Operation}
\newacronym{icnn}{ICNN}{Iterative Convolutional Neural Network}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{nn}{NN}{Neural Network}
\newacronym{nb}{NB}{Naive Bayesian}
\newacronym{mcs}{MCS}{Multiple Classifier System}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{ucnn}{$\mu$CNN}{Micro CNN}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Memristor (alphabetic order):								   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{brs}{BRS}{Bipolar Resistive Switch-based logic}
\newacronym{cnf}{CNF}{Conjunctive Normal Form}
\newacronym{crs}{CRS}{Complementary Resistive Switch-based logic}
\newacronym{dnf}{DNF}{Disjunctive Normal Form}
\newacronym{fpm}{FPM}{Forward Polarized Memristor}
\newacronym{hfo}{$HfO_x$}{Hafnium Oxide}
\newacronym{hrs}{HRS}{High Resistance State}
\newacronym{imc}{IMC}{In-Memory Computation}
\newacronym{imply}{IMPLY}{Material Implication Logic}
\newacronym{imp}{IMP}{In-Memory Processing}
\newacronym{lim}{LIM}{Logic in Memory}
\newacronym{lrs}{LRS}{Low Resistance State}
\newacronym{ltg}{LTG}{Logic Threshold Gate}
\newacronym{magic}{MAGIC}{Memristor-Aided Logic}
\newacronym{mecoins}{Me-Coin}{Memristor-based Computation In-memory}
\newacronym{pcm}{PCM}{Phase Change Memory}
\newacronym{pim}{PIM}{Processing in Memory}
\newacronym{reram}{ReRAM}{Resistive Random Access Memory}
\newacronym{rpm}{RPM}{Reversely Polarized Memristor}
\newacronym{stt}{STT}{Spin-transfer Torque}
\newacronym{tao}{$TaO_x$}{Tantalum Oxide}
\newacronym{tio}{$TiO_2$}{Titanium dioxide}
\newacronym{vteam}{VTEAM}{Voltage-controlled ThrEshold Adaptive Memristor}
\newacronym{team}{TEAM}{ThrEshold Adaptive Memristor}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Self-awareness (alphabetic order):						   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{aco}{ACO}{Autonomous Cooperating Object}
\newacronym{afdd}{AFDD}{Automated Fault Detection and Diagnostic}
\newacronym{ca}{CA}{Continuous Average}
\newacronym{cah}{CAH}{Context-Aware Health Monitoring}
\newacronym{cam}{CCAM}{Confidence-based Context-Aware condition Monitoring}
%\newacronym{cam}{C\textsuperscript{2}AM}{Confidence-based Context-Aware health Monitoring}
\newacronym[plural=DABs,longplural={Discrete Average Blocks}]{dab}{DAB}{Discrete Average Block}
\newacronym[plural=KPNs,longplural={Kahn Process Networks}]{kpn}{KPN}{Kahn Process Networks} 
\newacronym{mape-k}{MAPE-K}{Monitor-Analyze-Plan-Execute over a shared Knowledge}
\newacronym[plural=MoCs,longplural={Models of Computation}]{moc}{MoC}{Model of Computation}
\newacronym{oda}{ODA}{Observe-Decide-Act}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{rosa}{RoSA}{Research on Self-Awareness}
\newacronym{sa}{SA}{Self-Aware}
\newacronym{saness}{SA}{Self-Awareness}
\newacronym{sahm}{SAHM}{Self-Aware Health Monitoring}
\newacronym{samba}{SAMBA}{Self-Aware health Monitoring and Bio-inspired coordination for distributed Automation systems}
%\newacronym{sc}{SC}{Stability Controller}
\newacronym{sh}{SH}{State Handler}
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Systems (alphabetic order):								   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{cps}{CPS}{Cyber-Physical System}
\newacronym{cpps}{CPPS}{Cyber-Physical Production System}
\newacronym{dsr}{DSR}{Down-Sampling Rate}
\newacronym{dum}{DuM}{Device under Monitoring}
\newacronym{es}{ES}{Embedded System}
\newacronym{mes}{MES}{Manufacturing Execution System}
\newacronym{sc}{SC}{Stochastic Computing}
\newacronym{sos}{SoS}{System of Systems}
\newacronym{suo}{SuO}{System under Observation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% System on Chip (alphabetic order):						   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{abi}{ABI}{Application Binary Interface}
\newacronym{adc}{ADC}{Analog-to-Digital Converter}
\newacronym{aes}{AES}{Advanced Encryption Standard}
\newacronym{alu}{ALU}{Arithmetic Logic Unit}
\newacronym{api}{API}{Application Programming Interface}
\newacronym{asic}{ASIC}{Application Specific Integrated Circuit}
\newacronym{asoc}{ASOC}{Autonomic System-on-Chip platform}
\newacronym{axi}{AXI}{Advanced eXtensible Interface Bus}
\newacronym{bram}{BRAM}{Block Random Access Memory}
\newacronym{cdt}{CDT}{C/C++ Development Tooling}
\newacronym{clb}{CLB}{Configuarable Logic Block}
\newacronym{cmos}{CMOS}{Complementary Metal-Oxide Semiconductor}
\newacronym{cp}{CP}{Clock Pulse}
\newacronym{cpi}{CPI}{Cycles Per Instruction}
\newacronym{cpu}{CPU}{Central Processing Unit} 
\newacronym{cpsoc}{CPSoC}{Cyber-Physical System-on-Chip}
\newacronym{cu}{CU}{Compute Unit}
\newacronym{cuda}{CUDA}{Compute Unified Device Architecture}
\newacronym{dac}{DAC}{Digital to Analog Converter}
\newacronym{ddr3}{DDR3}{Double Data Rate}
\newacronym{dff}{DFF}{Data Flip-Flop}
\newacronym{dll}{DLL}{Delay Locked Loop}
\newacronym{dmr}{DMR}{Dual Modular Redundancy}
\newacronym{dram}{DRAM}{Dynamic Random Access Memory}
\newacronym{dsd}{DSD}{Digital Synchronous Detection}
\newacronym{dsp}{DSP}{Digital Signal Processor}
\newacronym{dt}{DigiTime}{}
\newacronym{dvfs}{DVFS}{Dynamic Voltage and Frequency Scaling}
\newacronym{eda}{EDA}{Electronic Design Automation}
\newacronym{fdc}{FDC}{Frequency-to-Digital Converter}
\newacronym{fifo}{FIFO}{First In First Out}
\newacronym{fpga}{FPGA}{Field Programmable Gate Array}
\newacronym{gds}{GDS}{Global Data Share}
\newacronym{gnulgpl}{GNU LGPL}{GNU Lesser General Public Licence} 
\newacronym{gpgpu}{GPGPU}{General Purpose Graphics Processing Unit}
\newacronym{gpr}{GPR}{General Purpose Register}
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{gro}{GRO}{Gated Ring Oscillator}
\newacronym{io}{IO}{Input-Output}
\newacronym{hamsoc}{HAMSoC}{Hierarchical Agent Monitoring System-on-Chip}
\newacronym{hdl}{HDL}{Hardware Description Language}
\newacronym{hmp}{HMP}{Heterogeneous Multi-Processor}
\newacronym{ic}{IC}{Integrated Circuit}
\newacronym{icap}{ICAP}{Internal Configuration Access Port}
\newacronym[longplural={Intellectual Properties}]{ip}{IP}{Intellectual Property}
\newacronym{isa}{ISA}{Instruction Set Architecture}
\newacronym{lds}{LDS}{Local Data Share}
\newacronym{lru}{LRU}{Least Recently Used}
\newacronym{lsb}{LSB}{Least-Significant Bit}
\newacronym{lsu}{LSU}{Load Store Unit}
\newacronym{lut}{LUT}{Look Up Table}
\newacronym{mash}{MASH}{Multi-Stage Noise-Shaping}
\newacronym{mems}{MEMS}{Micro-Electro-Mechanical Systems}
\newacronym{miaow}{MIAOW}{Many-core Integrated Accelerator Of deepwater/Wisconsin}
\newacronym{mosfet}{MOSFET}{Metal Oxide Semiconductor Field Effect Transistor}
\newacronym{mpsoc}{MPSoC}{Multi-Processor System-on-Chip}
\newacronym{mshr}{MSHR}{Miss Status Holding/Handling Register}
\newacronym{noc}{NoC}{Network-on-Chip}
\newacronym{opencl}{OpenCL}{Open Computing Language}
\newacronym{ocn}{OCN}{On-Chip Network}
\newacronym{pcb}{PCB}{Printed Circuit Board}
\newacronym{pcie}{PCIe}{Peripheral Component Interconnect Express}
\newacronym{pl}{PL}{Programmable Logic}
\newacronym{pli}{PLI}{Verilog Programming Language Interface}
\newacronym{pll}{PLL}{Phase-Locked Loop}
\newacronym{ps}{PS}{Processing System}
\newacronym{pv}{PV}{Process Variation}
\newacronym{qoe}{QoE}{Quality of Experience}
\newacronym{qos}{QoS}{Quality of Service}
\newacronym{ram}{RAM}{Random Access Memory} 
\newacronym{risc}{RISC}{Reduced Instruction Set Computer}
\newacronym{riscv}{RISC-V}{Reduced Instruction Set Computing - V}
\newacronym{rtl}{RTL}{Register-Transfer Level}
\newacronym{sdk}{SDK}{Software Development Kit}
\newacronym{seec}{SEEC}{SElf-awarE Computing}
\newacronym{sgpr}{SGPR}{Scalar General Purpose Register}
\newacronym{si}{SI}{Southern Island}
\newacronym{simd}{SIMD}{Single Instruction Multiple Data}
\newacronym{simf}{SIMF}{Single Instruction Multiple Floating point}
\newacronym{sm}{SM}{Streaming Multiprocessor}
\newacronym{snr}{SNR}{Signal-to-Noise Ratio}
\newacronym[plural=SoCs,firstplural=Systems on Chip (SoCs)]{soc}{SoC}{System-on-Chip}
\newacronym{spared}{SPARED}{Self-aware PArtial Reconfiguration architecture for Edge Devices}
\newacronym{spice}{SPICE}{Simulation Program With Integrated Circuit Emphasis}
\newacronym{tad}{TAD}{Time \gls{adc}}
\newacronym[plural=TDCs,longplural={Time-to-Digital Converters}]{tdc}{TDC}{Time-to-Digital Converter}
\newacronym{tq}{TQ}{Time-Quantizer}
\newacronym{uart}{UART}{Universal Asynchronous Receiver/Transmitter}
\newacronym{vcdu}{VCDU}{Voltage Controlled Delay Unit}
\newacronym{vco}{VCO}{Voltage Controlled Oscillator}
\newacronym{vga}{VGA}{Video Graphics Array}
\newacronym{vhdl}{VHDL}{Very High Speed Integrated Circuit Hardware Description Language}
\newacronym{vlsi}{VLSI}{Very Large Scale Integration}
\newacronym{vgpr}{VGPR}{Vector General Purpose Register}
\newacronym{xilffs}{XILFFS}{Generic Fat File System Library}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%General (uncategorized):									   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{amd}{AMD}{Advanced Micro Devices}
\newacronym{beol}{BEOL}{Back End Of Line}
\newacronym{cad}{CAD}{Computer-Aided Design}
\newacronym{cas}{CAS}{Circuits and Systems}
\newacronym{eu}{EU}{European Union}
\newacronym{fdd}{FDD}{fault detection and diagnostic}
\newacronym{fefet}{FeFET}{Ferroelectric Field Effect Transistor}
\newacronym{feline}{FeLINe}{FeFET Logic IN mEmory}
\newacronym[plural=FoMs,longplural={Figures of Merit}]{fom}{FoM}{Figure of Merit}
\newacronym{hipeac}{HiPEAC}{High Performance and Embedded Architecture and Compilation}
\newacronym{hp}{HP}{Hewlett Packard}
\newacronym{hqp}{HQP}{Highly Qualified People}
\newacronym{hvac}{HVAC}{Heating, Ventilation and Air Conditioning}
\newacronym{ibm}{IBM}{International Business Machines corporation}
\newacronym{ict}{ICT}{Institute for Computer Technology}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{nda}{NDA}{Non-Disclosure Agreement}
\newacronym{nvp}{NVP}{Non-Volatile Processor}
\newacronym{oecd}{OECD}{Organization for Economic Cooperation and Development}
\newacronym{rd}{R\&D}{Research and Development}
\newacronym{soa}{SoA}{State-of-the-Art}
\newacronym{tsmc}{TSMC}{Taiwan Semiconductor Manufacturing Company}
\newacronym{tvlsi}{TVLSI}{Transactions on Very Large Scale Integration}

\newacronym{cmp}{CMP}{Circuits Multi Project}
\newacronym{msb}{MSB}{Most-Significant Bit}
\newacronym{felix}{FELIX}{Fast and energy-efficient Logic in Memory}
\newacronym{esd}{ESD}{Electrostatic Discharge}
\newacronym{sdc}{SDC}{Self Directed Channel}
\newacronym{tmsl}{TMSL}{Three Memristors Stateful Logic}










